Optimal Sample Complexity of Contrastive Learning

Contrastive learning is a highly successful technique for learning representations of data from labeled tuples, specifying the distance relations within the tuple. We study the sample complexity of contrastive learning, i.e. the minimum number of labeled tuples sufficient for getting high generalization accuracy. We give tight bounds on the sample complexity in a variety of settings, focusing on arbitrary distance functions, both general $\ell_p$-distances, and tree metrics. Our main result is an (almost) optimal bound on the sample complexity of learning $\ell_p$-distances for integer $p$. For any $p \ge 1$ we show that $\tilde \Theta(\min(nd,n^2))$ labeled tuples are necessary and sufficient for learning $d$-dimensional representations of $n$-point datasets. Our results hold for an arbitrary distribution of the input samples and are based on giving the corresponding bounds on the Vapnik-Chervonenkis/Natarajan dimension of the associated problems. We further show that the theoretical bounds on sample complexity obtained via VC/Natarajan dimension can have strong predictive power for experimental results, in contrast with the folklore belief about a substantial gap between the statistical learning theory and the practice of deep learning.

==> result_old.tex <==
\section{$\ell_p$-distance}

Our proof uses a variant on a result in geometric probability \cite{W62}. In \cite{W62}, it is shown that the convex hull of $m$ uniformly random points on the unit sphere in $\mathbb{R}^n$ contains the point zero with probability exactly $2^{-m+1} \sum_{i=1}^{n-1} {m-1 \choose i}$. In Appendix \todo{ref}, we follow a similar proof to \cite{W62} in order to obtain the following theorem:

\begin{theorem}
\label{thm:geo_altered}
Let $v_1,\dots,v_m$ be a set of vectors on the unit sphere in $\mathbb{R}^n$, and let $s_1,\dots,s_m$ be i.i.d uniform random variables on $\{-1,1\}$. Then the convex hull of the set of random vectors $s_1 \cdot v_1,\dots, s_m \cdot v_m$ contains zero with probability at least $2^{-m+1} \sum_{i=1}^{n-1} {m-1 \choose i}$.
\end{theorem}

For a set of variables $x_1,\dots,x_n$ and functions $P_1,\dots,P_m$ such that $P_i:\mathbb{R}^n \rightarrow \mathbb{R}$ depending on variables $x_1,\dots,x_n$, denote by $\{P_i(x_1,\dots,x_n) \lessgtr 0\}_{i=1}^m$ as the random set of constraints containing i.i.d for each $i$ either  $P_i(x_1,\dots,x_n) > 0$ with probability $0.5$, or otherwise $P_i(x_1,\dots,x_n) < 0$.


%we add the constraint $\dist(x_i,y_i) > \dist(x_i,z_i)$ with probability $0.5$, and otherwise add $\dist(x_i,y_i) < \dist(x_i,z_i)$, for each $i$ independently.

\begin{corollary}
\label{cor:linear_equations_prob}
Let $P_1,\dots,P_m$ be linear combinations of $n$ variables $x_1,\dots,x_n$, i.e. $P_i(x_1,\dots,x_n) = \sum_{j=1}^n c_{i,j} x_j$, where $c_{i,j} \in \mathbb{R}$ is some constant for every $i \in [m],j \in [n]$. Let $C$ be the random set of linear inequalities $C = \{P_i(x_1,\dots,x_n) \lessgtr 0\}$. Then with probability at least $2^{-m+1} \sum_{i=1}^{n-1} {m-1 \choose i}$ on the choice of $C$, there is no assignment $(x_1,\dots,x_n) \in \mathbb{R}^n$ that satisfies $C$. 
\end{corollary}

Let $d \in \mathbb{N}$ be the dimension, and $V$ our element set. Assume we are given $m = \Omega(nd\log(n))$ triplets $M = \{(x_i,y_i,z_i)\}_{i=1}^m$ where each $x_i,y_i,z_i \in V$. For each triplet, we choose a labeling uniformly at random, i.e. $\vec{M} = \left\{ \dist(x_i,y_i) - \dist(x_i,z_i) \lessgtr 0 \right\}$. Our goal is to show that there exists a labeling of $M$ that cannot be satisfied in any embedding in $\mathbb{R}^d$. Let $\vec{M}$ be the set of resulting distance constraints.

An ordering is a set of functions $\pi_1,\dots,\pi_d$, where $\pi_i: V \rightarrow [n]$ is a one-to-one function. Given an embedding of $V = \{x_1,\dots,x_n\}$ into a set of points $P = \{p_1,\dots,p_n\} \subseteq \mathbb{R}^d$, we say that the embedding into $P$ satisfies the ordering $\pi_1,\dots,\pi_d$ if for any $i \in [d]$ and elements $x_j,x_\ell$ it holds that $p_j(i) < p_\ell(i)$ if and only if $\pi_{\ell}(p_j) > \pi_i(j)$. In other words, the embedding satisfies $\pi_1,\dots,\pi_d$ if for any $i$, the permutation $\pi_i$ determines the order of the elements of $V$ in the $i$'th dimension. For $x,y \in V$, we define $\pi_i(x,y) = 1$ if $x$ precedes $y$ in $\pi_i$, and otherwise $-1$.

Next, we show that with probability $1-\frac{1}{2^{\Omega(nd\log{n})}}$ for any given ordering functions $\pi_1,\dots,\pi_d$, the points of $V$ cannot be embedded while satisfying both the distance constraints $\vec{M}$ and the ordering $\pi_1,\dots,\pi_d$. The claim then follows from a union bound on all possible orderings.

\begin{lemma}
\label{lem:l1_fixed_permutation}
Let $\pi_1,\dots,\pi_d$ be an ordering. Then with probability at least $2^{-m+1} \sum_{i=1}^{n-1} {m-1 \choose i}$, any embedding of $v_1,\dots,v_n$ in $\mathbb{R}^d$ satisfying $\vec{M}$ does not satisfy the ordering $\pi_1,\dots,\pi_d$.
\end{lemma}
\begin{proof}
Let $\pi_1,\dots,\pi_d$ be an ordering. Then the set of constraints $\vec{M}$ is the set
$$\vec{M} = \left\{\sum_{j=1}^d \left(|x^j_i-y^j_i| - |x^j_i-z^j_i|\right) \lessgtr 0 \right\}.$$ 
If the embedding also satisfies the ordering $\pi_1,\dots,\pi_d$, then the embedding satisfies the constraint set
$$C = \left\{\sum_{j=1}^d \left(\pi_j(x_i,y_i)(x^j_i-y^j_i) - \pi_j(x_i,z_i)(x^j_i-z^j_i)\right)\lessgtr 0 \right\}.$$

By Corollary~\ref{cor:linear_equations_prob}, the constraint set $C$ is unsatisfiable with probability at least $p = 2^{-m+1} \sum_{i=1}^{n-1} {m-1 \choose i}$. In particular, with probability at least $p$, there is no embedding satisfying both $\vec{M}$ and the ordering $\pi_1,\dots,\pi_d$.
\end{proof}

The number of possible orderings is at most $(n!)^d \leq 2^{cnd\log{n}}$, for some constant $c > 0$. Recall we assume that $m=c'nd\log{n}$ for a sufficiently large $c' > 0$, therefore $2^{-m+1} \sum_{i=1}^{n-1} {m-1 \choose i} > 2^{cnd\log{n}}$. Therefore, by Lemma~\ref{lem:l1_fixed_permutation} and the union bound over all possible orderings, any embedding of $x_1,\dots,x_n$ in $\mathbb{R}^d$ satisfying $\vec{M}$ does not satisfy any ordering $\pi_1,\dots,\pi_d$. This implies that with probability greater than zero on the choice of $\vec{M}$, no embedding of $x_1,\dots,x_n$ satisfies $\vec{M}$. The claim follows.



\section{Upper bound for $\ell_1$-distance}

% \paragraph{Lower bound} Below, we prove that the VC dimension is at least $\Omega(nd)$.

% \begin{theorem}
%     For a dataset of size $n$ in dimension $d$, the VC-dimension of contrastive learning for $\ell_1$-distances is $\Omega(nd)$
%     \todo{Add minimum}
% \end{theorem}

% \begin{proof}

%     Consider the $d$ vectors $v_1, \dots, v_d$ corresponding to the rows of the Hadamard matrix.
%     The key property of these vectors is that for any subset $S$ which doesn't contain $i$ and any positive integer $c \ge |S|$:

%     \[\dist_1(c v_i, \sum_{j \in S} v_j) = cd\]

%     We select $d$ points and assign them to $p_{v_i} = D v_i$, where $D$ is a sufficiently large constant.
    
%     The remaining $n-d$ points are partitioned into a matching of size $\frac{n-d}{2}$.
%     We create queries of the form $(v_i, x, y)$ for every $i$ and every element $(x,y)$ in the matching.

%     We initialize the $n-d$ points at $0^d$ and build them iteratively.
%     For a query $(v_i, x, y)$, if $\dist_1(v_i, x) < \dist_1(v_i, y)$, then we update the point $p_x$ corresponding to $x$ to $p_x + v_i$.
%     Otherwise, we update the point $p_y$ corresponding to $y$ to $p_y + v_i$.

%     Let's fix $x$ and let $S$ be the set of all updates applied to $x$.
%     Then for any $v_i$ we have:
%     \[
%         \dist_1(p_{v_i}, p_x) = \dist_1(p_{v_i},\sum_{i \in S} v_i)
%     ,\]
%     where $S$ is the set of all updates which have been applied to $x$.
%     Notice that there that if just apply the $i$-th update on $x$ then $\dist_1(p_{v_i}, p_x) = (D - 1) d$ since $p_{v_i} - p_x = (D- 1) v_i$.
%     By the key property of Hadamard vectors above applying any other update for $j \neq i$ doesn't change the $\ell_1$ norm of this vector.
%     On the other hand, if query $(v_i, x, y)$ doesn't update $x$, then $p_{v_i} - p_y = D v_i$, where we again used the key property of the Hadamard vectors.
    
%     As a result, this set of queries is shattered.
%     Since there are $d$ vectors $v_1, \ldots, v_d$, and $\frac{n-d}{2}$ pairs formed from the remaining vectors, we proved that the VC dimension is at least $\Omega(d (n - d))$.
% \end{proof}


We first prove a simpler result for $d=1$ (i.e. when the points are on the line), which demonstrates the main technique.
Before that, we present the following useful lemma.

\begin{lemma}[A modified version of~\cite{W62}]
    \label{lem:hemisphere}
    Let $v_1, \ldots, v_m$ be vectors in a $n$-dimensional space.
    Let $s_1, \ldots, s_m$ be i.i.d. random variables with $s_i$ uniformly sampled from $\{-1, 1\}$.
    Then, the probability that the convex hull of $\{s_1 v_1, \ldots, s_m v_m\}$ doesn't contain the zero vector is at most $\frac{1}{2^{m-1}} \sum_{k=0}^{n-1} {m - 1 \choose k}$.
\end{lemma}
The proof is presented after the proof of Theorem~\ref{thm:one_dim_ub}.

\begin{theorem}
    \label{thm:one_dim_ub}
    For a dataset of size $n$, the VC-dimension of contrastive learning for $\ell_1$-distances (or, equivalently, $\ell_2$-distances) on a line ($d=1$) is $O(n \log n)$.
\end{theorem}

\begin{proof}
    Arranging points on the line puts them in a certain order.
    In our proof, we show that given $\Omega(n \log n)$ queries, for any fixed order, random labeling of the queries can't be satisfied by this order with probability at least $1 - \frac{1}{2 n!}$.
    Then, using union bound over all orderings, we get that random labeling can't be satisfied by any ordering with probability at least $\frac 12$, finishing the proof.
    
    Assume that the order of points on the line is fixed, and hence we know how all absolute values are resolved: i.e. $|x - y|_1 = x - y$ if $x$ is to the right of $y$ and $|x - y|_1 = y - x$ otherwise.
    Let the points be $V = \{x_1, \ldots, x_n\}$, and we want to fix their order: w.l.o.g. let $m:\ V \to \R$ be the arrangement of the points so that $m(x_1) < m(x_2) < \cdots < m(x_n)$.
    Then, let $\Delta_{i} = m(x_{i+1}) - m(x_i)$ for $i \in [n-1]$, and distance between points can be expressed in terms of $\{\Delta_i\}$, i.e. $x_{t} - x_{s} = \sum_{i=s}^{t-1} \Delta_i$ for $t > s$.
    
    In this notation, every labeled query $(x_i, x_j, x_k)$ corresponds to the inequality $|m(x_i) - m(x_j)| < |m(x_i) - m(x_k)|$, which becomes a linear inequality on $\{\Delta_i\}$.
    Moreover, labeled queries $(x_i, x_j, x_k)$ and $(x_i, x_k, x_j)$ (the positive and the negative sample are swapped) differ only in the sign of the inequality.

    We represent every inequality $\alpha_1 \Delta_1 + \ldots +\alpha_{n-1} \Delta_{n-1} < 0$ as a vector $(\alpha_1, \ldots, \alpha_{n-1})$.
    Note that changing the sign of the inequality is equivalent to multiplying the vector by $-1$.
    We denote these vectors as $v_1, \ldots, v_m$, and random labeling produces vectors $s_1 v_1, \ldots, s_m v_m$, where $s_i$ is uniformly sampled from $\{-1, 1\}$.

    Assume that there is a non-trivial non-negative linear combination of the vectors producing the zero vector, i.e. $\sum_{i=1}^m \beta_i s_i v_i = 0$ such that $\beta_i \ge 0$ for all $i$ and not all $\beta_i > 0$ for some $i$.
    In particular, a convex combination is always a non-trivial non-negative combination.
    In this case, we can sum the corresponding inequalities with multipliers $\{\beta_i\}$, and get inequality $0 < 0$, leading to a contradiction.
    Hence, if the zero vector lies in the convex hull, then the corresponding set of labeled queries can't be satisfied by the selected ordering.
    
    Finally, we use Lemma~\ref{lem:hemisphere} which says that the probability that the zero vectors lies in the convex hull is at least $1 - \frac{1}{2^{m-1}} \sum_{k=0}^{n-1} {m - 1 \choose k} \ge 1 - \frac{(1 + m)^n}{2^{m-1}}$, where $m$ is the number of queries.
    Since we want to union bound over all orders, we want to achieve $\frac{n! (1 + m)^n}{2^{m-1}} < \frac 12$.
    By choosing $m$ of form $c n \log n$ for some constant $c$, we have
    \[
        n \log n + n (\log c + \log (1 + n \log n)) + \log 2 < c n \log n - 1,
    \]
    which is satisfied for a sufficiently large $c$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:hemisphere}]
    First, note that it suffices to upper-bound the probability that the vectors lie in the same half-space going through $0$ (i.e. there is a vector $u$ such that $\InnerProd{u,s_i v_i} > 0$ for all $i \in [m]$).
    Indeed, if the zero vector doesn't lie in the convex hull, then such a half-space exists by the hyperplane separation theorem.

    Our proof that such a half-plane doesn't exist follows the general structure of~\cite{W62}, with the main difference being that we don't require the independence assumption~\footnote{\cite{W62} shows equality, but assumes that every subset of vectors of size at most $n$ is independent}.
    Let $p_{n,m}$ be the upper bound (over all possible vectors $v_1, \ldots, v_m$) on the probability that vectors lie in the same half-space.
    For each $i \in [m]$, let $A_i$ be the plane $\{x \mid \InnerProd{x,v_i}=0\}$.
    Let $S = \R^d \setminus \cup_{i=1}^m A_i$, i.e. the open set complementary to $\cup_{i=1}^m A_i$.
    This set consists of $K_{n,m}$ components separated by $A_i$'s, and in each component $C$ for each $i$ we have that the sign of $\InnerProd{u, v_i}$ is the same for all $u \in C$.
    These components correspond to the only choices of signs so that the vectors lie in the same half-space, and hence $p_{n,m} \le \frac{K_{n,m}}{2^{m}}$.

    It remains to prove that $K_{n,m} \le 2 \sum_{k=0}^{n-1} {m-1 \choose k}$
    Note that $K_{n,m} \le 2^m = 2 \sum_{k=0}^{m-1} {m-1 \choose k}$ for $m \le n$ and $K_{n,1} = 2 = 2 {0 \choose 0}$ for all $n$.
    Then, it suffices to prove that $K_{n,m} \le K_{n - 1,m - 1} + K_{n,m - 1}$, since then:
    \[
        \frac{K_{n,m}}{2}
        \le \sum_{k=0}^{n-2} {m-2 \choose k} + \sum_{k=0}^{n-1} {m-2 \choose k}
        = {m-2 \choose 0} + \sum_{k=1}^{n-1} {m-1 \choose k}
    \]
    
    Consider $S' = \R^d \setminus \cup_{i=1}^{m-1} A_i$, i.e. partition of $\R^d$ without the plane $A_m$.
    The number of components in $S'$ is at most $K_{n, m-1}$.
    There are two types of components in $S'$:
    \begin{itemize}
        \item Components not intersecting with $A_m$. These components result in only one component in $S= \R^d \setminus \cup_{i=1}^{m} A_i$.
        \item Components intersecting with $A_m$. These components result in two components in $S$.
    \end{itemize}
    Hence, the number of components in $S$ is at most the number of components in $S'$ (and there are at most $K_{n,m-1}$ of them) plus the number of components in $S'$ intersecting with $A_m$ (and we will show that there are at most $K_{n-1,m-1}$ of them).

    Let $B_i = A_i \cap A_m$ for $i \in [m-1]$.
    Clearly, $B_1, \ldots, B_{m-1}$ corresponds to a plane in $A_m$, and they partition $A_m$ into components corresponding to components in $S'$ cut by $A_m$.
    Since $A_m$ has dimension $n-1$, and there are $m-1$ planes $B_1, \ldots, B_{m-1}$, the number of such components is at most $K_{n-1, m-1}$.
    
    Hence, we proved the recurrent relation $K_{n,m} \le K_{n,m-1} + K_{n-1,m-1}$ and finished the proof.
\end{proof}
